ParallelBench: Understanding the Trade-offs of Parallel Decoding in Diffusion LLMs

While most autoregressive LLMs are constrained to one-by-one decoding, diffusion LLMs (dLLMs) have attracted growing interest for their potential to dramatically accelerate inference through parallel decoding. Despite this promise, the conditional independence assumption in dLLMs causes parallel decoding to ignore token dependencies, inevitably degrading generation quality when these dependencies are strong. However, existing works largely overlook these inherent challenges, and evaluations on standard benchmarks (e.g., math and coding) are not sufficient to capture the quality degradation caused by parallel decoding. To address this gap, we first provide an information-theoretic analysis of parallel decoding. We then conduct case studies on analytically tractable synthetic list operations from both data distribution and decoding strategy perspectives, offering quantitative insights that highlight the fundamental limitations of parallel decoding. Building on these insights, we propose ParallelBench, the first benchmark specifically designed for dLLMs, featuring realistic tasks that are trivial for humans and autoregressive LLMs yet exceptionally challenging for dLLMs under parallel decoding. Using ParallelBench, we systematically analyze both dLLMs and autoregressive LLMs, revealing that: (i) dLLMs under parallel decoding can suffer dramatic quality degradation in real-world scenarios, and (ii) current parallel decoding strategies struggle to adapt their degree of parallelism based on task difficulty, thus failing to achieve meaningful speedup without compromising quality. Our findings underscore the pressing need for innovative decoding methods that can overcome the current speed-quality trade-off. We release our benchmark to help accelerate the development of truly efficient dLLMs.

==> figures/results_block_size.tex <==
\begin{wrapfigure}{r}{0.32\textwidth}
\vspace{-\baselineskip}
    \centering
    %\includegraphics[width=1\linewidth]{dbench-figures-main/final_version/semi_ar_decoding/waiting_line_and_text_writing.pdf}
    \includegraphics[width=1\linewidth]{example-image}
    \caption{Semi-AR results on \textit{Text Writing} and \textit{Waiting Line}.}
    \label{fig:semi-ar}
\vspace{-\baselineskip}
\end{wrapfigure}


\begin{comment}

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.195\textwidth}
        \centering
        \includegraphics[width=\linewidth]{example-image}
        \caption{...}
        %\label{subfig:waiting_line_copy}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.195\textwidth}
        \centering
        \includegraphics[width=\linewidth]{dbench-figures-main/words_to_sentence/two_tokens_per_step/methods/random.pdf}
        \caption{...}
        %\label{subfig:waiting_line_reverse}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.195\textwidth}
        \centering
        \includegraphics[width=\linewidth]{example-image}
        \caption{...}
        %\label{subfig:waiting_line_replace_index}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.195\textwidth}
        \centering
        \includegraphics[width=\linewidth]{example-image}
        \caption{...}
        %\label{subfig:waiting_line_replace_random}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.195\textwidth}
        \centering
        \includegraphics[width=\linewidth]{example-image}
        \caption{...}
        %\label{subfig:waiting_line_shuffle}
    \end{subfigure}
    \caption{block size}
    \label{fig:results_block_size}
\end{figure}

\end{comment}

==> sec/reproducibility_statement.tex <==
\section*{Reproducibility Statement}

We provide an anonymous link to our code as a footnote in the abstract. The appendix provides further information on the dataset's creation and statistics (\cref{app:bench_data_details}).
